The SDSS-DR12 large-scale cross-correlation of Damped Lyman Alpha Systems with the Lyman Alpha Forest

We present a measurement of the DLA mean bias from the cross-correlation of DLA and the Ly$\alpha$ forest, updating earlier results of Font-Ribera et al. 2012 with the final BOSS Data Release and an improved method to address continuum fitting corrections. Our cross-correlation is well fitted by linear theory with the standard $\Lambda CDM$ model, with a DLA bias of $b_{\rm DLA} = 1.99\pm 0.11$; a more conservative analysis, which removes DLA in the Ly$\beta$ forest and uses only the cross-correlation at $r> 10{\rm h^{-1}\,Mpc}$, yields $b_{\rm DLA} = 2.00\pm 0.19$. This assumes the cosmological model from \cite{Planck2015} and the Ly$\alpha$ forest bias factors of Bautista et al. 2017, and includes only statistical errors obtained from bootstrap analysis. The main systematic errors arise from possible impurities and selection effects in the DLA catalogue, and from uncertainties in the determination of the Ly$\alpha$ forest bias factors and a correction for effects of high column density absorbers. We find no dependence of the DLA bias on column density or redshift. The measured bias value corresponds to a host halo mass $\sim 4\cdot10^{11} {\rm M_{\odot}}$ if all DLA were hosted in halos of a similar mass. In a realistic model where host halos over a broad mass range have a DLA cross section $\Sigma(M_h) \propto M_h^{\alpha}$ down to $M_h > M_{\rm min} =10^{8.5} {\rm M_{\odot}}$, we find that $\alpha > 1$ is required to have $b_{\rm DLA}> 1.7$, implying a steeper relation or higher value of $M_{\rm min}$ than is generally predicted in numerical simulations of galaxy formation.

==> glossary.tex <==
\setacronymstyle{long-short}
\glssetnoexpandfield{first}
\glssetnoexpandfield{firstpl}

\newglossaryentry{2dF}{
	type={acronym},
	name={2dF Survey},
	description={Two-degree-Field Galaxy Redshift survey},	
	first={\glsentrytext{2dF}},
}

\newglossaryentry{AGN}{
	type={acronym},
	name={AGN},
	description={Active Galactic Nuclei},
	descripcio={galàxia de nucli actiu},
	first={\glsentrydesc{AGN} (\glsentrytext{AGN})},
}

\newglossaryentry{BAL}{
	type={acronym},
	name={BAL},
	description={Broad Absorption Line},	
	first={\glsentrydesc{BAL} (\glsentrytext{BAL})},
	plural={BALs},
	descriptionplural={Broad Absorption Line},
	firstplural={\glsentrydescplural{BAL} (\glsentryplural{BAL})},
}

\newglossaryentry{BAO}{
	type={acronym},
	name={BAO},
	description={Baryon Acoustic Oscillations},
	descripcio={oscil·lacions acústiques dels barions},
	first={\glsentrydesc{BAO} (\glsentrytext{BAO})},
}

\newglossaryentry{BBN}{
	type={acronym},
	name={BBN},
	description={Big Bang Nucleosynthesis},
	descripcio={nucleosíntesi primordial},
	first={\glsentrydesc{BBN} (\glsentrytext{BBN})},
}

\newglossaryentry{BI}{
	type={acronym},
	name={BI},
	description={balnicity index},
	first={\glsentrydesc{BI} (\glsentrytext{BI})},
}

\newglossaryentry{BOSS}{
	type={acronym},
	name={BOSS},
	description={Baryon Oscillations Spectroscopic Survey},
	first={\glsentrydesc{BOSS} (\glsentrytext{BOSS})},
}

\newglossaryentry{CDM}{
	type={acronym},
	name={CDM},
	description={Cold Dark Matter},
	descripcio={matèria fosca freda},
	first={\glsentrydesc{CDM} (\glsentrytext{CDM})},
}

\newglossaryentry{CFHTLenS}{
	type={acronym},
	name={CFHTLenS},
	description={a lensing catalogue},
	first={\glsentrytext{CFHTLenS}},
}

\newglossaryentry{CMASS}{
	type={acronym},
	name={CMASS},
	description={a catalogue of ``constant mass" luminous infrared galaxies from \gls{BOSS}},
	first={\glsentrytext{CMASS}},
}

\newglossaryentry{CMB}{
	type={acronym},
	name={CMB},
	description={Cosmic Microwave Background},
	descripcio={fons còsmic de microones},
	first={\glsentrydesc{CMB} (\glsentrytext{CMB})},
}

\newglossaryentry{CNR}{
	type={acronym},
	name={CNR},
	description={continuum-to-noise ratio},
	first={\glsentrydesc{CNR} (\glsentrytext{CNR})},
}

\newglossaryentry{COBE}{
	type={acronym},
	name={COBE},
	description={COsmic Background Explorer},
	first={\glsentrytext{COBE}},
}

\newglossaryentry{DE}{
	type={acronym},
	name={DE},
	description={dark energy},
	first={\glsentrydesc{DE} (\glsentrytext{DE})},
}

\newglossaryentry{DLA}{
	type={acronym},
	name={DLA},
	description={Damped \lya{} Absorber},
	descripcio={sistema \lya{} esmorteïta},
	descripcioplural={sistemes \lya{} esmorteïts},
	descriptionplural={Damped \lya{} Absorbers},
	first={\glsentrydesc{DLA} (\glsentrytext{DLA})},	
	plural={DLAs},
	firstplural={\glsentrydescplural{DLA} (\glsentryplural{DLA})},
}

\newglossaryentry{DM}{
	type={acronym},
	name={DM},
	description={dark matter},
	first={\glsentrytext{DM}},
}

\newglossaryentry{DR}{
	type={acronym},
	name={DR},
	description={Data Release},
	first={\glsentrydesc{DR} (\glsentrytext{DR})},
}

\newglossaryentry{DRXQ}{
	type={acronym},
	name={DRXQ},
	description={\ifglsused{DR}{DRX quasar catalogue}{Data Release 9 quasar catalogue\glsunset{DR}}},
}

\newglossaryentry{DR7}{
	type={acronym},
	name={DR7},
	description={seventh Data Release},
	first={\ifglsused{DR}{\glsentrytext{DR7}}{\glsentrydesc{DR7} (\glsentrytext{DR7}) \glsunset{DR}}},
}

\newglossaryentry{DR9}{
	type={acronym},
	name={DR9},
	description={ninth Data Release},
	first={\ifglsused{DR}{\glsentrytext{DR9}}{\glsentrydesc{DR9} (\glsentrytext{DR9}) \glsunset{DR}}},
}

\newglossaryentry{DR9Q}{
	type={acronym},
	name={DR9Q},
	description={DR9 quasar catalogue},
	first={\ifglsused{DRXQ}{\glsentrytext{DR9Q}}{\ifglsused{DR}{\glsentrydesc{DR9Q} (\glsentrytext{DR9Q})}{\glsentrydesc{DR9} quasar catalogue (\glsentrytext{DR9Q})}\glsunset{DRXQ}\glsunset{DR}}},
}
	
\newglossaryentry{DR10}{
	type={acronym},
	name={DR10},
	description={tenth Data Release},
	first={\ifglsused{DR}{\glsentrytext{DR10}}{\glsentrydesc{DR10} (\glsentrytext{DR10}) \glsunset{DR}}},
}

\newglossaryentry{DR11}{
	type={acronym},
	name={DR11},
	description={eleventh Data Release},
	first={\ifglsused{DR}{\glsentrytext{DR11}}{\glsentrydesc{DR11} (\glsentrytext{DR11}) \glsunset{DR}}},
}

\newglossaryentry{DR12}{
	type={acronym},
	name={DR12},
	description={twelfth Data Release},
	first={\ifglsused{DR}{\glsentrytext{DR12}}{\glsentrydesc{DR12} (\glsentrytext{DR12}) \glsunset{DR}}},
}

\newglossaryentry{DR12Q}{
	type={acronym},
	name={DR12Q},
	description={DR12 quasar catalogue},
	first={\ifglsused{DRXQ}{\glsentrytext{DR12Q}}{\ifglsused{DR}{\glsentrydesc{DR12Q} (\glsentrytext{DR12Q})}{\glsentrydesc{DR12} quasar catalogue (\glsentrytext{DR12Q})}\glsunset{DRXQ}\glsunset{DR}}},
}

\newglossaryentry{FLRW}{
	type={acronym},
	name={FLRW},
	description={Friedmann–Lema\^itre–Robertson–Walker},
	first={\glsentrydesc{FLRW} (\glsentrytext{FLRW})},
}

\newglossaryentry{FRW}{
	type={acronym},
	name={FRW},
	description={Friedmann–Robertson–Walker},
	first={\glsentrydesc{FRW} (\glsentrytext{FRW})},
}

\newglossaryentry{GR}{
	type={acronym},
	name={GR},
	description={general relativity},
	descripcio={relativitat general},
	first={\glsentrydesc{GR} (\glsentrytext{GR})},
}
	
\newglossaryentry{HCD}{
	type={acronym},
	name={HCD},
	description={high-column-density system},
	descriptionplural={high-column-density systems},
	first={\glsentrydesc{HCD} (\glsentrytext{HCD})},	
	plural={HCDs},
	firstplural={\glsentrydescplural{HCD} (\glsentryplural{HCD})},
}
	
\newglossaryentry{IGM}{
	type={acronym},
	name={IGM},
	description={intergalactic medium},
	descripcio={medi intergalàctic},
	first={\glsentrydesc{IGM} (\glsentrytext{IGM})},
}

\newglossaryentry{LCDM}{
	type={acronym},
	name={$\Lambda$CDM},
	description={$\Lambda$ Cold Dark Matter},
	first={\ifglsused{CDM}{\glsentrytext{LCDM}}{\glsentrydesc{LCDM} (\glsentrytext{LCDM}) \glsunset{CDM}}
},
}

\newglossaryentry{LSS}{
	type={acronym},
	name={LSS},
	description={large-scale structure},
	first={\glsentrydesc{LSS} (\glsentrytext{LSS})},
}

\newglossaryentry{MJD}{
	type={acronym},
	name={MJD},
	description={Modified Julian Date},
	first={\glsentrydesc{MJD} (\glsentrytext{MJD})},
}

\newglossaryentry{MTC}{
	type={acronym},
	name={MTC},
	description={\textit{Mean Transmission Correction} },
	first={\glsentrydesc{MTC} (hereafter \glsentrytext{MTC})},
}

\newglossaryentry{PSF}{
	type={acronym},
	name={PSF},
	description={Point Spread Function},
	first={\glsentrydesc{PSF} (\glsentrytext{PSF})},
}

\newglossaryentry{RMS}{
	type={acronym},
	name={RMS},
	description={root mean square},
	first={\glsentrydesc{RMS} (\glsentrytext{RMS})},
}

\newglossaryentry{SDSS}{
	type={acronym},
	name={SDSS},
	description={Sloan Digital Sky Survey},
	first={\glsentrydesc{SDSS} (\glsentrytext{SDSS})},
}

\newglossaryentry{SDSS-II}{
	type={acronym},
	name={SDSS-II},
	description={Sloan Digital Sky Survey II},
	first={\ifglsused{SDSS}{\glsentrytext{SDSS-II}}{\glsentrydesc{SDSS-II} (\glsentrytext{SDSS-II})  \glsunset{SDSS}}},
}

\newglossaryentry{SDSS-III}{
	type={acronym},
	name={SDSS-III},
	description={Sloan Digital Sky Survey III},
	first={\ifglsused{SDSS}{\glsentrytext{SDSS-III}}{\glsentrydesc{SDSS-III} (\glsentrytext{SDSS-III})  \glsunset{SDSS}}},
}

\newglossaryentry{SN}{
	type={acronym},
	name={SN},
	description={supernova},
	descriptionplural={supernovae},
	descripcio={supernova},
	descripcioplural={supernoves},
	first={\glsentrydesc{SN} (\glsentrytext{SN})},
	plural={SNe},
	firstplural={\glsentrydescplural{SN} (\glsentryplural{SN})},
}

\newglossaryentry{WMAP}{
	type={acronym},
	name={WMAP},
	description={Wilkinson Microwave Anisotropy Probe},
	first={\glsentrytext{WMAP}},
}


==> src/DLA_discussion_mod.tex <==

%________________________SECTION________________________%
%
\section{Discussion}  \label{sec DLA: Discussion}

%_______________subsection_______________%
\subsection{Systematic errors: Cross-correlation modelling}
\label{subs DLA: systematics}

 So far, all of the errors we have quoted for $b_{\rm DLA}$ include only
statistical errors of the cross-correlation measurement, computed either
from our covariance matrix or the bootstrap analysis. We now discuss
systematic errors, which arise from two sources: uncertainties in the
model of the cross-correlation to be used in the fit, and impurity of
the \gls*{DLA} sample. We discuss first the modelling uncertainties.

 There are several possible sources of systematic error of $b_{\rm DLA}$
in our modelling procedure: the continuum fitting correction, the assumed
cosmological model, the use of linear theory, the \lya{} bias factors,
and the \gls*{HCD} correction. We believe our continuum fitting correction is
accurate, in view of the good agreement of two independent methods of
applying this correction from FR12 and the distortion matrix procedure
used here (see section \ref{subs DLA: distortion}), and the tests that
have been made with mocks \citep{Bautista+2017}. While we have shown
that there is a high sensitivity to the cosmological model (a 10\%
variation of $b_{\rm DLA}$ is caused by the update from the WMAP model
of FR12 to the Planck model we use), this does not cause a large
systematic if we believe that the results of \cite{Planck2015} are
accurate. As we shall see below, we are particularly interested in
systematics that might lower our inferred value of $b_{\rm DLA}$, to
bring it in closer agreement with expectations from cosmological
simulations of galaxy formation, and this can only occur by further
increasing $\sigma_8(z_{\rm ref})$ or $\Omega_m$ in the cosmological
model. Linear theory seems well justified from the constant value of
$b_{\rm DLA}$ with scale (figure \ref{fig DLA: dla bias dependence r})
and the large value of $r_{\rm min}$ we are using, although precise
predictions of non-linearities in the \gls*{DLA}-\lya{} cross-correlation from
cosmological simulations would be highly desirable to test this.

  We believe the more important sources of systematics are in the
uncertainties in the \lya{} bias factors and the \gls*{HCD} correction
determined from the \lya{} autocorrelation. If we use the two models
fitted to the \lya{} autocorrelation in \cite{Bautista+2017}, the
'Ly$\alpha$' one in their table 5 without \gls*{HCD} correction and
$\beta_{\rm Ly\alpha}=1.246$, and the full model in their table 3 with
\gls*{HCD} correction and $\beta_{\rm Ly\alpha}=1.663$, the difference
of $\sim$ 5\% in the implied $b_{\rm DLA}$ between the two models is a
good estimate of our systematic error, which is comparable to our
statistical error of $b_{\rm DLA}$. The model including the \gls*{HCD}
correction gives the lowest value of $b_{\rm DLA}$, and we
conservatively take it as our final result to compare with predictions
from galaxy formation simulations. The statistical errors in the \lya{}
bias factors of the models of \cite{Bautista+2017} are negligibly small
for our purpose.

  We note that even though the \gls*{HCD} correction is not a very
accurate representation of the true effect of \glspl*{HCD}, since it
does not take into account the precise Voigt profile shape of the
absorbers, we believe the important thing is that the same model that
provides a good fit to the measured \lya{} autocorrelation is used to
model the \gls*{DLA}-\lya{} cross-correlation.

%_______________subsection_______________%
\subsection{Systematic errors: Sample Purity and Selection}
\label{subs DLA: purity samples}

 We now discuss the purity and selection effects of our samples A, C1 and C2.
\Glspl*{DLA} are detected using the automatic algorithm described in
\cite{Noterdaeme+2009,Noterdaeme+2012b}, which searches for regions of
strong absorption that are consistent with a damped \lya{} absorption
line plus the random absorption by the \lya{} forest. We therefore expect
that some fraction of these candidate \glspl*{DLA} in the catalogue are
not real \glspl*{DLA}, and are likely to be instead regions of strong absorption
over a sufficiently broad velocity interval to look approximately like a
damped profile, but with a real HI column density much less than
$10^{20}\, {\rm cm}^{-2}$. These false detections should increase at low
$N_{\rm HI}$ and low signal-to-noise. For very low signal-to-noise some
false \glspl*{DLA} may not correspond to any absorber but be mostly
caused by noise, but these cases should be rare with our imposed
cut of $CNR > 3$.

 The fact that we observe no variation of $b_{\rm DLA}$ with column
density suggests that the effect of these contaminants on $b_{\rm DLA}$
is not large. Either the impurity is too small to affect our result, or
the false \glspl*{DLA} are regions of absorption with a bias that is close to
that of \glspl*{DLA}. An additional argument against a large level of
impurity of our sample is the result of \cite{Mas-Ribas+2016} on the
dependence of the mean equivalent width of high-ionization lines of \glspl*{DLA}
on $N_{\rm HI}$ (see their figure 11), which varies only by 20\% over
the available range of column densities. Moreover, this small variation
is not necessarily due to a variation of the impurity level, but can be
caused by a real physical effect.

 A more detailed study requires predicting the purity of our catalogue
using \lya{} forest mock spectra. This is not a simple calculation,
because the mock spectra must have the correct distribution of \glspl*{HCD} with
broad absorption features that can mimic \glspl*{DLA} (which our current mocks
are not designed to reproduce), and \glspl*{DLA} must be inserted in the mock
spectra with the correct cross-correlation, so we leave this for future
studies.

 Different issues arise with \glspl*{DLA} detected blueward of the \lyb{} quasar
emission line, where the \lyb{} forest is superposed with \lya{}
absorption and the possibilities of confusion increase. Often, a DLA may
be detected in part because there is a \lyb{} line from an absorber that
has most of the column density, resulting in an incorrect assigned
redshift. In the absence of any real \lya{} absorber, these absorbers
with incorrect redshifts should contribute a zero cross-correlation to
our measurement, decreasing the fitted value of $b_{\rm DLA}$ by a
fractional amount equal to the fraction of these systems. Our sixth
cut, applied to define sample A, eliminates these misidentified objects,
which are therefore present only in our samples C1 and C2
(see section \ref{sec DLA: Sample data}; sample C1 is the largest, due to
not including cuts 4 and 5 that eliminate \glspl*{DLA} too close to the \ovi{} and
\lya{} quasar emission lines).

 For $r_{\rm min}=5\hmpc$, we measure $b_{\rm DLA} = 2.06 \pm
0.11$ for sample A, $b_{\rm DLA}=1.97\pm 0.08$ for sample $C1$, and
$b_{d} = 1.99\pm 0.09$ for sample C2. These errors are obtained from
our covariance matrix, and are roughly proportional to the inverse
square root of the number of \glspl*{DLA} in each sample. The variation in the
bias of the \gls*{DLA} samples is hardly significant, especially if the
larger bootstrap errors are considered (see table \ref{ta DLA: biases}),
although they go in the expected direction of a decreased $b_{\rm DLA}$
in samples with an expected higher impurity. This suggests that
\glspl*{DLA} removed by cuts 4 to 6 are primarily \glspl*{DLA} or other
absorption systems with a similar bias factor.

\begin{figure*}
	\centering
	\includegraphics[width=0.7\textwidth]{lyb_corr.eps}
	\caption{\gls*{DLA} transmission spectrum of the total sample of
\protect\cite{Mas-Ribas+2016} (black line), and the same transmission
spectrum for the larger sample including \glspl*{DLA} in the \lyb{} forest
region, which may include \lyb{} absorbtion lines misidentified as \lya{}
lines of \glspl*{DLA} (thick, red line). The absorption feature at
$\sim 1,441\angs$ suggests that these misidentified \glspl*{DLA} are
$\sim$ 1\% of the sample.}
	\label{fig DLA: lyb contamination}
\end{figure*}

 The level of impurity due to \lyb{} absorption lines confused by \lya{}
n samples C1 and C2 can also be estimated by stacking the absorption
spectra. If a \lyb{} absorption line is incorrectly attributed to \lya{}
absorption at $\lambda_\alpha=1216\, {\rm \AA}$, then the true \lya{}
absorption will appear at $32/27 \lambda\alpha=1441\, {\rm \AA}$.
Figure \ref{fig DLA: lyb contamination}) shows the stacked spectrum
obtained with the technique of \cite{Mas-Ribas+2016} for what was
designated as ``total sample'' by these authors, which excluded \glspl*{DLA}
found in the \lyb{} forest region, as the black line. The red line is
the stacked spectrum of the larger sample including \glspl*{DLA} in the \lyb{}
forest region, and shows the expected absorption of misidentified
absorbers at a level of $\sim $ 1\% . We take this as an upper limit to
the fraction of systems in our C1 and C2 samples that are \lyb{} lines
wrongly identified as \lya{} lines of \glspl*{DLA}, because these \lyb{} lines
are more likely to be identified when they have superposed true \lya{}
absorption. This indicates that this contamination of the sample is
very small and not significant compared to our statistical errors.

 In general, the inclusion of any false absorbers in our catalogue arising
purely from noise or from misidentified redshifts can only decrease our
measured $b_{\rm DLA}$, because the false absorbers have a null average
contribution to the cross-correlation. The presence of \gls*{HCD} absorbers
misidentified as \glspl*{DLA} may increase our measured bias only if the \gls*{HCD}
bias is higher than that of \glspl*{DLA}. There is, however, a systematic
arising from a selection effect that may increase the measured
$b_{\rm DLA}$, already mentioned in FR12: if \glspl*{DLA} are more likely to be
detected when the \lya{} forest that is superposed with their damped
wings is weaker than average, then this would preferentially select \glspl*{DLA}
surrounded by high-density large-scale regions, over those in low
density regions. The reason is that the \gls*{DLA}-\lya{} cross-correlation is
negative along the line-of-sight at $\left| r_\parallel \right| \gtrsim 20 \hmpc$
owing to redshift space distortions, implying weaker \lya{} forest
absorption over the damped wings of \glspl*{DLA} in more overdense regions.
This is a selection effect that can only be properly corrected with the
use of adequate mock spectra with \glspl*{DLA} inserted with the correct
cross-correlation with the \lya{} forest. Again, we believe this
correction is unlikely to be large because of the absence of dependence
of $b_{\rm DLA}$ on $N_{\rm HI}$, but future studies will need to better
address this question.

%_______________subsection_______________%
\subsection{Evolution of the bias factor} \label{subs DLA: bias evolution}

 The lack of a significant dependence of $b_{\rm DLA}$ on redshift and
column density was shown for sample A in figure
\ref{fig DLA: dla bias dependence}, although a large scatter was noticed
for the redshift dependence for the case with $r_{\rm min}=10\hmpc$,
with a lower bias for the middle redshift than the low and high redshift
ones by $\sim 2.5\sigma$. To explore if this scatter might indicate
something other than noise, we repeat the measurement using sample C1,
taking into account that decreased purity is unlikely to be very
important as argued in section \ref{subs DLA: purity samples}.

\begin{table}
	\centering
	\begin{tabular}{cr}
		\toprule
		Name & Number of \glspl*{DLA} \\
		\midrule
		ZC1	& 6,319\\
		ZC2 	& 6,664\\
		ZC3	& 10,359\smallskip\\
		NC1	& 8,613\\
		NC2	& 7,788\\
		NC3	& 6,941\\
		\bottomrule
	\end{tabular}
	\caption{Number of DLAs in the subsamples ZC1 to ZC3 and NC1 to
NC3, drawn from sample C1.}
	\label{ta DLA: sample properties extended}
\end{table}

  We define six new subsamples by dividing the C1 sample into the same
three redshift and column density bins as in table
\ref{ta DLA: sample properties} for sample A. The number of systems in the
new subsamples are shown in table \ref{ta DLA: sample properties extended},
nearly doubling those from sample A.
Results are shown in figure \ref{fig DLA: dla bias dependence}, where
squares with dashed error bars show the bias
values obtained with the new subsamples, and the circles with
solid error bars show the previous results from sample A. The normal
scatter for sample C1 suggests that the anomalously high scatter
in sample A is only due to statistical noise.

The fact that no change of the bias factor (within 10\%) is seen between redshift 2 to 3 suggests that the characteristic host halo mass is decreasing with redshift. The independence with column density also suggests that the mean NHI radial profile is similar in host halos of different masses. 



%_______________subsection_______________%
\subsection{Implications on the distribution of DLA host halo masses}
\label{subs DLA: halo mass}

 The bias factor of dark matter halos as a function of their mass is
robustly predicted in analytic models and numerical simulations
\citep[see e.g.][]{Sheth+1999, Tinker+2010}, and therefore our derived
DLA bias factor implies a condition on the characteristic mass of halos
hosting \glspl*{DLA}. We use the model of \citet{Tinker+2010} to
calculate the halo bias at the mean redshift of our cross-correlation
measurement $z=2.3$, shown as the thick solid curve in figure
\ref{fig DLA: dla halo mass} (both left and right panels). The grey
horizontal line with the shaded band is the value of $b_{\rm DLA}$ for
our C1 sample and $r_{\rm min} = 5\hmpc$, with the bootstrap error. This
is the result with the smallest error that we believe we can trust, as
we have argued above. However, it does not include the systematic error
arising mainly from the \lya\ bias factors and impurities in the catalog.

 If all \glspl*{DLA} were in halos with a single value of the mass, the
inferred halo mass would be placed from $2.5\cdot 10^{11}\hmsun$ to
$5\cdot 10^{11}\hmsun$ given our statistical error bar, corresponding
to a massive galaxy. However, in any realistic model, \glspl*{DLA}
host halos should have a broad mass range. Our measurement yields only
the mean bias factor, which depends on the \gls*{DLA} cross section as a
function of halo mass as discussed in FR12. This cross section depends
on the distribution of gas in halos, and therefore on the complex
physics of gas accretion, galaxy formation, and galactic and quasar
winds that can expel gas from a central galaxy to the outer regions of
halos or to the intergalactic medium.

  Following FR12, we assume a power-law distribution of the DLA
cross-section $\Sigma(M_h)$ as a function of halo mass,
\begin{equation}
	\label{eq DLA: DLA cross-section} 
	\Sigma(M_h) = \Sigma_{0}\left(\frac{M_h}{M_{\rm min}}\right)^{\alpha}
\,\,\,\,\left(M>M_{min}\right)~,
\end{equation}
The predicted mean DLA bias under this simple assumption is
\begin{equation}
 b_{\rm DLA} = { \int_{M_{\rm min}}^{M_{\rm max}}
  n(M_h) \Sigma(M_h) b(M_h)\, dM_h
 \over \int_{M_{\rm min}}^{M_{\rm max}} n(M_h) \Sigma(M_h) \, dM_h } ~,
\end{equation}
where $n(M_h)$ is the number density and $b(M_h)$ the bias of
halos of mass $M_h$. We have also assumed that the cross section is
negligible below a minimum mass $M_{\rm min}$ and above a maximum mass
$M_{\rm max}$. Numerical simulations of galaxy formation including
hydrodynamics and complex recipes for star formation and galaxy winds
driven by supernova explosions have been extensively studied by several
groups 
%\citep[e.g.,][]{Pontzen+2008,Tescari+2009,Bird+2014}}, 
(e.g., Pontzen et al. 2008; \DIFaddbegin \DIFadd{Tescari et al. 2009;} \DIFaddend Bird et al. 2014)
and can predict this
relationship. In particular, \cite{Bird+2014} find a relation that is
well fitted by a power-law over the halo mass range that can be probed
by their simulations, $10^{8.5}\hmsun < M < 10^{12}\hmsun$. At lower
masses, the intergalactic photoionized gas has sufficient pressure to
slow the accretion onto halos. At higher halo masses, the small box
of their simulations do not allow enough halos to be included to derive
solid predictions.

\begin{figure*}
	\centering
	\includegraphics[width=\textwidth]{fig14Font-Ribera12_newcosmo.pdf}
	\caption{{\it Left:} Average \gls*{DLA} bias when the
\protect\gls*{DLA} cross-section as a function of halo mass
follows the power-law relation in equation (\ref{eq DLA: DLA cross-section}),
for the indicated values of the power-law index $\alpha$, as a function
of the lower mass cutoff $M_{\rm min}$.
{\it Right:} Same as in the left panel but including an upper mass
cutoff at $M_{max}=10^{13}\hmsun$. The bias for a single halo mass is shown
in both panels as the thick solid line. All cases are computed at
$z = 2.3$. Horizontal shaded region is our derived value for the
\gls*{DLA} bias (sample C1, $r_{\rm min}=5\hmpc$) and the 1$\sigma$
statistical bootstrap error (not including errors on the \lya{} forest
bias factors).}
	\label{fig DLA: dla halo mass}
\end{figure*}

  The mean DLA bias computed in this model is shown in the left panel of
figure \ref{fig DLA: dla halo mass} as a function of $M_{\rm min}$, and
in the limit of infinite $M_{\rm max}$, for six different values of the
power-law index $\alpha$. For $M_{min}=10^{8.5}\hmsun$, the required
slope to match our DLA bias is $\alpha\sim 1.1$. The simulations of
\cite{Bird+2014} tend to give a lower slope of $\alpha\simeq 1.0$, which
corresponds to $b_{\rm DLA}\simeq 1.7$ for the same value of
$M_{\rm min}$, which is discrepant with our measurement at the
$\sim 2-\sigma$ level if we use only our statistical, bootstrap errors,
but may be more consistent with what we measure when including plausible
systematic errors from uncertainties in the \lya\ forest bias factors
and the effects of catalog impurity. If a bias factor $b_{\rm DLA} >
1.9$ is confirmed by future by improved determinations, then either a
steeper slope or higher value of $M_{\rm min}$ compared to the
\cite{Bird+2014} simulations would be required. Results of earlier
simulations that had weaker galactic winds and predicted slopes of
$\alpha\simeq 0.7$ \citep{Pontzen+2008}, with much lower implied DLA
bias factors of $b_{\rm DLA} < 1.5$, are strongly ruled out by our
measurement. In general, the high value of $b_{\rm DLA}$ we measure
implies that the structure of DLAs is affected by strong galactic
winds, which are able to decrease the cross sections in low-mass halos
by expelling gas to the intergalactic medium, and increase cross
sections in high-mass halos by spreading gas out to large radius.

 However, \cite{Bird+2014} assumed an extrapolation of their power-law
fit to $M_h > 10^{12} \hmsun$ to derive a bias factor
$b_{\rm DLA}\simeq 1.7$ from their fitted power-law slope, because their
small simulations cannot predict the properties of the rare, more
massive halos. These massive halos are very highly biased and make an
important contribution to the mean bias of DLAs. The right panel of
figure \ref{fig DLA: dla halo mass} shows the same models using now an
upper cutoff $M_{\max}=10^{13} \hmsun$, and we see that in this case,
the predicted bias factor for $M_{\rm min}=10^{8.5} \hmsun$ and
$\alpha=1$ already decreases to $b_{\rm DLA}\simeq 1.6$. The results of
\cite{Bird+2014} can therefore agree with our measurement at better than
$2-\sigma$ only if we allow for a systematic error and if there is no
substantial flattening of the slope of the $\Sigma(M_h)$ relation at
$M_h > 10^{12} \hmsun$. There are reasons to expect this flattening of
the slope because at low redshift, we observe that massive halos are
associated with galaxy groups and clusters containing most of the
baryons in X-ray emitting hot gas, where much of the cold gas in
galaxies is destroyed owing to tidal and ram-pressure stripping
\citep{Fabian2012}. However, at the redshifts where \glspl*{DLA} in
\gls*{BOSS} are found, the amount of cold gas in very massive halos is
not well known. Larger and better simulations, and observations of
galaxy clusters at high redshift, are required to clarify this question.

 Our improved measurement of the bias factor of \glspl*{DLA} has an
impact on forecasts for 21-cm surveys of HI galaxies \citep[see, e.g,][]{Chang+2010,Chang+2015}: a higher
value of the bias implies a larger amplitude of the 21-cm
fluctuations. Our new value is very similar to the previous one by FR12,
with a reduced error and a more detailed analysis of model dependences.
The 21-cm fluctuation amplitude depends on the mean bias of all
absorbers weighted by their HI column density. The lack of dependence of
$b_{\rm DLA}$ on $N_{\rm HI}$, and the fact that most of the known
neutral hydrogen in the Universe resides in DLAs, strongly suggest that
our derived value $b_{\rm DLA}\simeq 2.0$ should apply for the neutral
gas that will be detected in 21-cm surveys. Although these surveys
should include dust-absorbed systems that are not included in our DLA
sample and lower column density systems that we also do not include, it
is difficult that these systems may change the mean bias factor
appreciably.

 Finally, we comment on one theoretical aspect of the bias of dark matter
halos that may influence the comparison of the theoretically predicted
and observed DLA bias factor. The halo bias is not only a function of
mass, but also of the assembly history of a halo, a phenomenon known as
``assembly bias'' \citep[e.g.,][]{Borzyszkowski+2017}. Halos of a fixed
mass in high-density regions tend to have accreted their mass recently,
whereas in low-density regions the accretion rate is lower. The DLA
cross section may depend also on the accretion history: for a fixed halo
mass, a high accretion rate may imply more atomic gas is available at
large radius to give rise to a DLA system, and at the same time a higher
bias owing to the assembly bias effect. This effect may be missed by
simulation results like those in \cite{Bird+2014} when the bias factor
is inferred from the DLA host halo mass distribution and the same type
of theoretical relation of bias and halo mass we have used here, instead
of being directly obtained from the simulation. 
\DIFaddbegin \DIFadd{Alternatively one may achieve a steeper slope cross-correlation - halo mas relation, and then get a higher predicted DLA bias, by changing some parameters of the winds models in simulation.
}\DIFaddend Future studies should
therefore also attempt to include the effect of assembly bias \DIFaddbegin \DIFadd{or wind model }\DIFaddend when
comparing to the observational result.

==> src/DLA_linear_theory_limits.tex <==
%________________________SECTION________________________%
%
\section{Limits on the linear theory}  \label{sec DLA: LT limits}
As discussed in \vref{sec DLA: Model} we are assuming that our measurements (or more precisely the part of the measurements used in the fitting process) are in the linear regime. As previously stated it is not clear which is the smallest distance at which we can safely assume the linear regime. The aim of this appendix is not to find such a limit, but to convince the reader that the ranges considered here are indeed in the linear regime or that, at least, the deviations from the linear regime are small. 

In order to do so, we explore the dependence of the model on the minimum distance considered for the analysis. We fit the model considering $r_{\rm min}=4\hmpc$, $r_{\rm min}=5\hmpc$, $r_{\rm min}=6\hmpc$, $r_{\rm min}=7\hmpc$, $r_{\rm min}=8\hmpc$, $r_{\rm min}=9\hmpc$, and $r_{\rm min}=10\hmpc$ for sample A. Even though the fits are performed using all the bins in $\sigma$, here we only show the first six bins in $\sigma$ as an example (see \vref{fig DLA: TL limits}; note that only the cases with $r_{\rm min}=4\hmpc$, $r_{\rm min}=6\hmpc$, $r_{\rm min}=8\hmpc$, and $r_{\rm min}=10\hmpc$ are plotted). The values of the fitted parameters are listed in \vref{ta DLA: TL limits}. While there are discrepancies between the models of a few \%, the measured bias is consistent between the models even though there seems to be a systematic decrease on the bias with $r_{\rm min}$. The reduced $\chi^{2}$ is roughly the same for the different models.


\begin{table}
	\centering
	\begin{tabular}{ccc}
	\toprule
	$r_{\rm min}\left(\hmpc\right)$	& $b_{d}$ & $\chi^{2} (d.o.f.)$ \\
	\midrule
	4	& $1.87 \pm 0.05$ & 2970.37 (2898-2)	\\
	5	& $1.88 \pm 0.05$ & 2965.22 (2896-2)	\\
	6	& $1.88 \pm 0.06$ & 2951.99 (2888-2)	\\
	7	& $1.88 \pm 0.06$ & 2958.96 (2888-2) \\
	8	& $1.89 \pm 0.07$ & 2951.60 (2878-2) \\
	9	& $1.89 \pm 0.07$ & 2944.27 (2874-2) \\
	10	& $1.90 \pm 0.08$ & 2939.15 (2864-2)	\\
	\bottomrule
	
	\end{tabular}
	\caption{Measured bias of the \gls{DLA} when fitting the same model but cutting at different $r_{min}$.}
	\label{ta DLA: TL limits}	
\end{table}

\begin{figure}
	\centering
	\includegraphics[width=0.45\textwidth]{test_linear_regime_plot_sigma_bin_0.eps}
	\includegraphics[width=0.45\textwidth]{test_linear_regime_plot_sigma_bin_1.eps}
	\includegraphics[width=0.45\textwidth]{test_linear_regime_plot_sigma_bin_2.eps}
	\includegraphics[width=0.45\textwidth]{test_linear_regime_plot_sigma_bin_3.eps}
	\includegraphics[width=0.45\textwidth]{test_linear_regime_plot_sigma_bin_4.eps}
	\includegraphics[width=0.45\textwidth]{test_linear_regime_plot_sigma_bin_5.eps}
	\caption[Measurement of the cross-correlation for different bins in $\sigma$. The values of $\sigma$ are expressed in $\hmpc$. In all panels blue circles are for sample A. Blue solid line, green dashed-dotted line, black dotted line, and red dashed line correspond to the best-fit model considering $r_{\rm min}=4\hmpc$, $r_{\rm min}=6\hmpc$, $r_{\rm min}=8\hmpc$, and $r_{\rm min}=10\hmpc$ respectively. Bottom panels show the ${\rm r}^{2}$-weighted differences between the different models and the best-fit model considering $r_{\rm min}=10\hmpc$.]{Measurement of the cross-correlation for different bins in $\sigma$: from left to right $0\hmpc<\sigma<4\hmpc$, $4\hmpc\le\sigma<8\hmpc$, $8\hmpc\le\sigma<12\hmpc$, $12\hmpc\le\sigma<16\hmpc$, $16\hmpc\le\sigma<20\hmpc$, $20\hmpc\le\sigma<28\hmpc$. The values of $\sigma$ are expressed in $\hmpc$. In all panels blue circles are for sample A. Blue solid line, green dashed-dotted line, black dotted line, and red dashed line correspond to the best-fit model considering $r_{\rm min}=4\hmpc$, $r_{\rm min}=6\hmpc$, $r_{\rm min}=8\hmpc$, and $r_{\rm min}=10\hmpc$ respectively. Bottom panels show the ${\rm r}^{2}$-weighted differences between the different models and the best-fit model considering $r_{\rm min}=10\hmpc$.}
	\label{fig DLA: TL limits}
\end{figure}
